Adapt3R: Adaptive 3D Scene Representation for Domain Transfer in Imitation Learning

Imitation Learning can train robots to perform complex and diverse manipulation tasks, but learned policies are brittle with observations outside of the training distribution. 3D scene representations that incorporate observations from calibrated RGBD cameras have been proposed as a way to mitigate this, but in our evaluations with unseen embodiments and camera viewpoints they show only modest improvement. To address those challenges, we propose Adapt3R, a general-purpose 3D observation encoder which synthesizes data from calibrated RGBD cameras into a vector that can be used as conditioning for arbitrary IL algorithms. The key idea is to use a pretrained 2D backbone to extract semantic information, using 3D only as a medium to localize this information with respect to the end-effector. We show across 93 simulated and 6 real tasks that when trained end-to-end with a variety of IL algorithms, Adapt3R maintains these algorithms' learning capacity while enabling zero-shot transfer to novel embodiments and camera poses.

==> figures/real_tasks_tex.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/real_tasks.pdf}
    \caption{Our real-world multitask imitation learning benchmark includes 6 pick-and-place tasks shown above.}
    \label{fig:real_tasks}
\end{figure}


==> figures/vis-attn-map.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.3\textwidth]{figures/images/attn_maps/reference.pdf}
        \caption{Scene Reference}
        \label{fig:attn-reference}
    \end{subfigure}
    

    \begin{subfigure}[b]{\textwidth}
        \centering
        % First Column
        \begin{tikzpicture}
            \node[anchor=south west, inner sep=0] (image1) at (0,0) {
                \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/alph-ref-27.png}
            };
            \begin{scope}[x={(image1.south east)},y={(image1.north west)}]
                \node[anchor=north] at (0.5, 1.1) {\textbf{Pre-Grasp PC}};
            \end{scope}
        \end{tikzpicture}
        % Second Column
        \begin{tikzpicture}
            \node[anchor=south west, inner sep=0] (image2) at (0,0) {
                \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/alph-attn-27.png}
            };
            \begin{scope}[x={(image2.south east)},y={(image2.north west)}]
                \node[anchor=north] at (0.5, 1.1) {\textbf{Pre-Grasp Attn. Map}};
                \draw[red, thick] (0.4, 0.32) rectangle (0.55, 0.52);
            \end{scope}
        \end{tikzpicture}
        % Third Column
        \begin{tikzpicture}
            \node[anchor=south west, inner sep=0] (image3) at (0,0) {
                \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/alph-ref-147.png}
            };
            \begin{scope}[x={(image3.south east)},y={(image3.north west)}]
                \node[anchor=north] at (0.5, 1.1) {\textbf{Post-Grasp PC}};
            \end{scope}
        \end{tikzpicture}
        % Fourth Column
        \begin{tikzpicture}
            \node[anchor=south west, inner sep=0] (image4) at (0,0) {
                \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/alph-attn-147.png}
            };
            \begin{scope}[x={(image4.south east)},y={(image4.north west)}]
                \node[anchor=north] at (0.5, 1.1) {\textbf{Post-Grasp Attn. Map}};
            \end{scope}
        \end{tikzpicture}
    
        \caption{``Move the alphabet soup to the basket"}
        \label{fig:attn-alph}
    \end{subfigure}

    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/milk-ref-10.png}
        \begin{tikzpicture}
            \node[anchor=south west, inner sep=0] (image) at (0,0) {
                \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/milk-attn-10.png}
            };
            \begin{scope}[x={(image.south east)},y={(image.north west)}]
                % Adjust the coordinates of the rectangle
                \draw[red, thick] (0.33, 0.22) rectangle (0.48, 0.52);
            \end{scope}
        \end{tikzpicture}
        \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/milk-ref-73.png}
        \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/milk-attn-73.png}
        \caption{``Move the milk to the basket"}
        \label{fig:attn-milk}
    \end{subfigure}

    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/oj-ref-33.png}
        \begin{tikzpicture}
            \node[anchor=south west, inner sep=0] (image) at (0,0) {
                \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/oj-attn-33.png}
            };
            \begin{scope}[x={(image.south east)},y={(image.north west)}]
                % Adjust the coordinates of the rectangle
                \draw[red, thick] (0.3, 0.25) rectangle (0.42, 0.57);
            \end{scope}
        \end{tikzpicture}
        \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/oj-ref-129.png}
        \includegraphics[width=0.23\textwidth]{figures/images/attn_maps/oj-attn-129.png}
        \caption{``Move the orange juice to the basket"}
        \label{fig:attn-oj}
    \end{subfigure}
    
    \caption{\todo{get rid of this figure, replace with new, better attention maps} In this figure we present visualizations of the attention maps at various points during execution for several tasks in the scene shown in (a). Specifically, the tasks are: (b) ``Move the alphabet soup to the basket", (c) ``Move the milk to the basket", and (d) ``Move the orange juice to the basket". For each task we provide (from left to right) a reference point cloud before the end effector has grasped the desired object, the corresponding attention map, a reference point cloud after grasping and while moving towards the basket, and the corresponding point cloud. We also draw a red box around the object the end effector will manipulate to help readers interpret the attention maps. In general we see that while the robot is moving towards the object, it pays more attention to the points corresponding to the object. While moving towards the basked it pays more attention to the basket. We provide videos of these in the ``attention maps'' folder of the supplementary material.}
    \label{fig:attn-maps}
\end{figure*}

